To Patch, or not To Patch? That is the Question: A Case Study of System Administrators' Online Collaborative Behaviour

System administrators, similar to end users, may delay or avoid software patches, also known as updates, despite the impact their timely application can have on system security. These admins are responsible for large, complex, amalgamated systems and must balance the security related needs of their organizations, which would benefit from the patch, with the need to ensure that systems must continue to run unimpeded. In this paper, we present a case study which follows the online life-cycle of a pair of Microsoft patches. We find that communities of sysadmins have evolved sophisticated mechanisms to perform risk assessments that are centred around collecting, synthesizing, and generating information on patches. These communities span different Virtual Communities of Practice, as well as influencers who monitor and report on the impact of new patches. As information is propagated and aggregated across blogs, forums, web sites, and mailing lists, eventually resulting in a consensus around the risk of a patch. Our findings highlight the role that these communities play in informing risk management decisions: Patch information is not static, and it transforms as communities collaborate to understand patch issues.

==> Submission_Reviews/CSCW_Review.tex <==

Reviewer 3 (1AC)
Review
This paper tracks down and reports on the sysadmin community’s reaction to a pair of patches from Microsoft (one security-only patch, and its matching cumulative patch). The paper traces reactions to the patches from a large sysadmin forum and an associated set of blogs as they discover issues with the patch, try to alert others about these issues, receive a “hot fix” that itself has issues, watch that hot fix get pulled, and then finally receive a working patch.

The paper tries to frame this as tracking a “community of practice”, but this theoretical framing is confused in the paper. The paper uses at least four related terms — community of practice, networked community of practice, virtual community of practice, and network of practice — but doesn’t define or explain these. There is no literature review about communities of practice or justification that this is such a community. There is little connection to the communities of practice literature, of which there is much in CSCW and beyond. The theoretical framing of this paper is weak.
1AC Recommendation to Editors
Reject
1AC meta-review
All of the reviewers found the paper to be relatively well written and to tell a interesting and informative story about a single patch. However, all three reviewers were concerned that this paper was a case study, and it wasn’t clear what we can learn from this case that goes beyond this specific case (which was a relatively arbitrarily chosen case). The methodology for choosing the case was presented, but the reasoning for that methodology was not; having more explicit reasoning would help justify what we are learning. The paper also tried to use a “communities of practice” theoretical lens for the paper, but that lens was confusing and did not help the readers to understand what can be learned from this case.

There was also concern from R2 that the paper was too long for the contribution. R1 also had a similar concern, saying that the paper was long because of the story, but the length did not match the contribution.
Reviewer 1 (Reviewer)
Recommendation(s) to 1AC
Reject
Review
Paper Summary and Contributions:
This paper provides an in-depth case study of two related Microsoft patches, through manually sifting through the posts and links in sysadmin mailing lists and forums discussing these patches. They track the chronology of events and the sentiments expressed in the posts. Their case study highlights how information flows between these different sources and how sysadmins operate within a broader online community that can both provide information and assistance with the patching process.

Paper Contribution’s Importance/Novelty and Execution:
Understanding how updating information propagates among the sysadmin community is relevant and important for the CSCW and security audience. The story presented in the paper is informative and I appreciate the insights one gains from the story.

However, this paper’s contribution is ultimately limited. The case study on only 2 rather unique patches (which are directly related to each other) specifically for Windows, considering a subset of mailing lists and forums, does not provide generalizable knowledge. We cannot determine whether the observations are common or anomalous. Furthermore, the analysis seems rather adhoc instead of a systematic process; many of the descriptions and conclusions from the paper are subjective and not grounded in the actual data, or extrapolate overly broadly from a single post. For example, Sec 5.1 says the announcements/curated lists help provide the necessary info in a single source. While this seems plausible, there’s no evidence of this from the data, and it is technically speculation. In general, the availability of certain information for sysadmins doesn’t necessarily indicate they know about, that they use it, or that they find it helpful. Similarly, Sec 5.6 identifies a couple posts expressing dissatisfaction with Microsoft pulling the hotfix and extrapolates this to betrayal of trust among sysadmins. The paper would be strengthened by expanding to more case studies, rigorously analyzing the data itself for deriving findings, and discussing how those findings provide guidance on future directions for the research or sysadmin community.

Paper Length: The paper seemed an appropriate length given it told a story in detail. However, I would recommend the authors focus on more case studies and the common events/components across them, rather than the nitty-gritty details for this particular timeline.
Reviewer 2 (Reviewer)
Recommendation(s) to 1AC
Major Revision
Review
This paper presents a case study of how sysadmins create and disseminate information that helps them to decide whether and when to apply patches. The authors selected two (paired and mutually exclusive) patches released by Microsoft on a “Patch Tuesday”, and illustrate how these patches are discussed on different online forums, and how decisions to wait or to patch are formed.

Strengths:
- Interesting and relevant theme
- Mostly well written (with small language mistakes)
- The paper has a certain arc of suspense, making it an interesting read

Weaknesses:
- I’m not sure how much the CSCW community can learn from a description of a single case
- Data collection seems to be limited (which the authors acknowledge)

The paper presents a chronological order of events that follow the release of a monthly Microsoft patch -- more precisely, a pair of patches that repair the same security issues and should be applied in a mutually exclusive way. The authors rigorously explain why they selected these particular patches for their analysis, and provide a rich description of online publications and discussions that followed the patch releases and the issues that they caused.

I certainly learned some new and interesting information from this paper, but I’m not quite sure that this is enough to warrant a publication as a full paper. That is, the amount of new findings seems to be more appropriate for a short paper. I feel that a paper analyzing several cases would be more preferable, maybe detailing which kinds of various issues might happen with the patches, and how they are resolved.

Moreover, data collection seems limited, as the authors used only snowballing from the mailing list Patchmanagement.org. The authors acknowledge this in the Limitations, but it is not clear how a simple web search for the analyzed patches would have changed the findings, and why the authors did not conduct a web search additionally to the snowballing.

While I can see the merits of this paper as it is, I think that these merits might be too low for a full paper, and the authors might need to extend the paper in two ways:

1) Additional search for the materials related to the patches (not only snowballing)
2) Several case studies, maybe highlighting issues that exhibit different communication and collaboration patterns

Minor issues: The paper has small mistakes and needs proofreading. Examples:
- and the Equifax data breach [cite]
- Sysadmins requires more investigation
- The struggles of end-users and updates is comparatively well explored when compare to sysadmins
and patching

==> Submission_Reviews/Rebuttals_Reviews.tex <==
We would like to begin by thanking all of the reviewers for their insightful and constructive comments. We aim to address the major comments that appeared across the reviews, however we will address all concerns highlighted such as formatting, and grammatical errors. An information flow graphic is under development and will be included and figure clarity will be improved.

System Admins Definition, Context and Framing (R-A, R-B, R-D):
We will add context about community composition. PatchManagement.org involves email addresses so we can provide a sense of the types of organizations represented. While the composition of the other groups is not easily obtained, we will clarify how the communities self-identify online. We will also clarify that community members likely have a wide range of duties from administering a large number of computers to managing a small businesses, or even self-administering. We also argue that these communities are regularly used. For example, PatchManagement.org represents around 5K unique email addresses, which indicates the scale of the community, while AskWoody.com has a global ALEXA rank of 123,396. For comparison, ieee-security.org ranks 376,502.

Approach and Implications (R-A, R-B, R-D):
Online communities are interesting to study in security because they accurately reflect the information being shared, rather than relying on self-report. Studying such communities of practice is regularly used in other fields, such as health, to understand the type of information medical professional share among themselves. 

For implications, we agree that the discussion needs improvement. We will add actionable intelligence for stakeholders (Reviewers A, D, C) by including discussion of the implications for sysadmins, developers, and researchers. For example, the issue of information "watering holes" such as StackOverflow have been highly discussed in developer centered security of late and we feel that a similar discussion needs to be happening around security advice communities aimed at admins. Our work provides an initial look into patch management information watering holes. 

Challenging to Generalize:
All authors noted that our case is challenging to generalize, which is a known limitation of case studies. However, they also provide an in-depth understanding at a level not possible to achieve in larger sample approaches, such as surveys, and are thus a needed element of early-stage research (Yin, R.K., 2017. Case study research and applications: Design and methods). 
The value of a case study comes from the systematic analysis of sources that, as R-C mentioned, could theoretically be found via Google Search. We extracted a cohesive  sequence of events that is contextualized within the patch process, and identified relevant theory that can be used to drive further investigation. 

We also note that organizations handle patch management very differently. Similar to R-B, we have also observed that admins at large organizations tend to test patches in-house. However, many admins do not have access to those resources, or want to learn about potential problems before testing. Our goal is to represent this community, not all admins. We will clarify this point.

==========
Final soups rebuttal is above. 

%Noted by R-B, large organizations would have the means and resources to focus internally, however this is possibly not the case for those in smaller institutions. R-A is correct too about tech-savvy users, but we argue this information is valuable in risk assessing patches, and is a component of these communities knowledge exchange.  

%While our information could theoretically be located via Google Search (R-C) we argue that the research value here comes from collecting these sources together and presenting them as a cohesive contextualized sequence of events, and relating the information to the patch process. 



We will elaborate on the importance of studying virtual communities for cyber security (R-B)
by detailing the benefits of such a lens by discussing research in the Health domain regarding the importance of virtual communities of practice. We argue that understanding how these social systems work could lead to cultivation of such communities, potentially improving overall security understanding. 
We will develop our findings to accommodate actionable intelligence for stakeholders (Reviewers A, D, C), by including discussion of the implications for sysadmins, developers, and researchers. For example, researchers could use our case study as the basis of exploring information sharing in Cyber Security, and how we can better connect the right information to the right groups. Potential lessons for admins include suitability of patch management strategies such as the potential use of AGILE methodologies. We will discuss our future work, which includes in-depth ethnographic studies of patching within varying organizations around Patch Tuesday.  

===========================================================================
Review #105A
===========================================================================

Overall merit
-------------
3. Weak accept: While flawed, the paper has merit and we should consider
   accepting it.

Suitability for SOUPS
---------------------
3. Suitable

Paper summary
-------------
The authors present a case study of patching behavior, as extrapolated from online forum posts for two Microsoft patches. The authors analyzed several different forums and specific influencers in the patch world.

Strengths
---------
The paper was an interesting read for me and I learnt a lot of background information on how administrators exchange information and what problems they face.
In particular I found the separation of some forums into a,b and w groups interesting.
The authors chose the patches well. Since Microsoft bungled both the patch and how they retracted the patch.

Weaknesses
----------
While the paper was a pleasant read, I am not sure what the actionable intelligence is that the reader will take from it.
I think it would have been a good idea to also include a non-bungled patch in the analysis. As it is the paper shows a worst case case-study.
The paper could also have been made stronger by contacting some of the admins and gathering further data from them.

Comments for authors
--------------------
Is it possible to differentiate between sys-admins and interested/tech-savvy end-users? Some of the quotes sound like they could come from users with only their personal machine.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105B
===========================================================================

Overall merit
-------------
1. Reject: This paper is well below the bar for SOUPS. Will argue to reject
   it.

Suitability for SOUPS
---------------------
3. Suitable

Paper summary
-------------
This paper examines the decision making process of system administrators as they determine the appropriate time to install security patches to their systems. The authors used a case study approach following a pair of updates through their lifecycle in online forums.

Strengths
---------
The paper is interesting and easy to read. The approach to the case study (in essence an audit log of what transpired in online communities once a patch was released) is non-traditonal and provides a unique perspective on patch management.

Weaknesses
----------
While the paper describes in detail the relationship between a number of online communities in the patch management space, it is not clear who is using this information and what community of sys admins are using the information to make decisions on patching or not.  Therefore it is difficult to determine the significance of the contribution and how it impacts the field of knowledge.  I am not sure what the traffic/messages and volume of data say about real decisions to patch or not or even if they have any influence.

How can this result -- the use of virtual communities improve the cyber security landscape.  This goes directly to the authors interest in this area " the lack of academic literature on this subject and the call for extending the field's focus".  Maybe there should be a stronger connection to improving the performance or need of sys admins in this patch space.

First and foremost how are system administrators defined and the context in which they work matters.  It is not clear who is providing information to these communities, are they home users, sys admins of big organizations/corporations/academic institutions/government or other orgs as well as who is using this data.  Size and capabilities of the org in addition to capabilities of the org,  all of these factors matter.  It would be very helpful to define the characteristics of those who are both providing input to these forums and those who are using the input.  Given just a small reach out to system admins in a couple of large orgs that I am familiar with, the sys admins had never heard of most of these communities and were surprised that anyone would follow them or take advice from them.  In addition they were concerned about taking security advice from unknown entities posting information.

Section 4 enumerates key communities and influencers, yet in section 5 other communities are discussed including Ghacks and the Zero Day Initiative.  How were the communities in section 4 identified and why not others?

Comments for authors
--------------------
Methodologically, I have a couple of comments. The authors "decided to analyze the data from process and information flow perspective".  Given that I would expect a diagram or flow chart of the data and the flows with timing data or at least a diagram of the chronology of events.  The sections are quite detailed but interspersed among the flows and chronology are  observations and discussion points. It would be preferable for section five to provide the data and section 6 to provide the observation of trust and the information economy perspective and others. 

The paper needs a thourough  read for typos and formatting.  For example section 2.1 first sentence The fist, and wee in section 5.9.  Formatting in section 5.2 bottom of page 8.  And the figures are very difficult to read even with reading glasses see figure 2 and 3.


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105C
===========================================================================

Overall merit
-------------
2. Weak reject: The paper has flaws, but I will not argue against it.

Suitability for SOUPS
---------------------
3. Suitable

Paper summary
-------------
The paper presents an online lifecycle of a couple of Microsoft patches. It shows how sysadmins have key influencers and online communities that help them decide when to install a patch and when to wait.

Strengths
---------
The paper tells a compelling story by looking at two patch releases from Microsoft, on how system administrators go to key sites and influencers on the internet to learn if they should wait or install the update. The authors present the timelines of these chosen incidents, when patches were problematic, they were withdrawn by Microsoft, and later rerelesed.

Weaknesses
----------
Nothing in this paper seems to be research. All the information presented (though said as a nice story), is basically accessible through Google search. The paper does not deliver on the promise in the abstract.

The two incidents chosen, though rich in events, might not be representative of how patch releases and installations usually go.

Comments for authors
--------------------
Page 4, section 4 presents "Key communities, influencers and companies". A discussion would be useful to justify how these key websites were identified.


Page 2: "The fist investigation" --> "The first investigation"


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #105D
===========================================================================

Overall merit
-------------
3. Weak accept: While flawed, the paper has merit and we should consider
   accepting it.

Suitability for SOUPS
---------------------
3. Suitable

Paper summary
-------------
The authors present a case study about the decision making process of system administrators when it comes to system updates. In their study, they analysed the decision making process between key influencers and the online community. The study focuses on two Microsoft patches which were released in 2017. The results indicate that there is a very active online community which is influenced by a few important key players. The results help to further understand the complexity of software update decision in system administration.

Strengths
---------
- the paper deals with a very important topic. An admin's decision to patch or not to patch influences the security and usability of many end users.

- the approach is novel and interesting. It can provide real-world insights into a very complex ecosystem.

- the paper is very well written and easy to understand. The related work is very well covered.

Weaknesses
----------
- It is not clear if and how the results can be generalised to a bigger population.

- The paper lacks actionable results. What do the results implicate for researchers, admins, and software developing companies?

Comments for authors
--------------------
I'd like to thank the authors for submitting this paper to SOUPS19. I would argue that the topic is highly relevant and that the paper provides important insights into a very complex ecosystem. Indeed, studying system administrators is a highly complex task and the authors' approach seems novel and reasonable. While I overall enjoyed reading this paper, I identified some aspects which should be addressed to further improve the submission.

The paper is well written and easy to read. I agree with the authors that the investigation of a focused but detailed problem can lead to more general insights about the administrators' processes and problems. While I did not find specific flaws in the study, I felt that the authors need to provide a more thoughtful discussion of the findings. I specifically wondered what we can learn about decision making of administrators in general. How can the investigated process be generalised to other groups of administrators or other software manufactures? I know that there is not "one" type of admins, but that is why I would appreciate a discussion. Do Server admins have the same problems as admins for work stations? Does Microsoft provide similar processes as Apple? Which general lessons can we learn from this case study?

In addition, I would appreciate if the authors could add some thoughts on the implications of their findings. What can the different stakeholders learn from this study?

Admins: Is the current process of making update decisions optimal or should better approaches be used (in theory)?

Researchers: Should we research ways to support the decision making? (e.g., by better connecting the communities virtually). On which aspect should we focus next? (E.g., to interview admins or key players about this process)

Software developers: What needs to be changed in the update process to make update decisions easier? (Do the authors have any ideas in addition to "more transparency/information").

While I enjoyed reading this paper, I would argue that the authors could make a better job in discussion the results. At the moment, the reader is almost left alone with the interpretation of the findings. I would like to learn about the three (more general) lessons learned we can draw from this well performed case study.

==> Text/Background.tex <==
%\paragraph{Patch Management}\footnote{\url{http://eddiejackson.net/web_documents/The_Administrator_Shortcut_Guide_to_Patch_Management.pdf}} 
%In the modern world, many organizations rely heavily on their computing resources to carry out critical work related to the success of the business. The management of these systems entails many processes to maintain a working and secure system. Arguably, the most important practice utilised to achieve this is that of Patch Management [cite CyberEssentials]. Patch management is a continuous process of applying patches or updates to system software and firmware to 'plug' potential vulnerabilities. Gerace and Cavusoglu identified the critical elements in the patch management process as~\cite{Gerace2009TheCE}:
%\begin{itemize}
%    \setlength\itemsep{-.2em}
%    \item Senior executive support, 
%    \item Dedicated resources and clearly defined responsibilities,
%    \item Creating and maintaining a current technology inventory, 
%    \item Identification of Vulnerabilities and Patches, 
%    \item Scanning and monitoring the network, 
%    \item Pre-deployment testing of patches, and
%    \item Post-deployment scanning and monitoring.
%\end{itemize}
%5Patch management dependent tasks rely on teams of sysadmins'  understanding of their systems. Armed with this  knowledge, admins are able to prepare their systems for potential patch deployments, as well as identify risks to their system's health. This step is continuously adaptive, as admins must maintain an up-to-date knowledge of known vulnerabilities, detailed available patch knowledge, company resource management, and evaluations of patch process efficiency. Furthermore, with every new patch applied to a system, their is the potential to reevaluate their, already restricted~\cite{hrebec2001survey}, understandings of the systems they manage. 
%The second phase focuses primarily on reliably establishing when new patches are deployed, parsing the details, and pinpointing the patches which relate to their systems' unique make-up. 
%Once the correct patches have been identified, sysadmins must trawl through large amounts of related patch information, such as the severity of the patch's vulnerability, to decide the necessity of a patch, allowing them to structure and plan the appropriate amount of resources to complete the patch deployment. This stage also includes the testing of the patch on a production-like environment in order to gauge the patches' suitability. Since patches are often built with time restrictions, they can be deployed with imperfections. Testing allows sysadmins to mitigate the potential damage that patches can cause to business critical elements of their systems.
%The final phase is to deploy the patch to all intended systems, rolling out to the production environment, once the patch is considered 'safe'. However, this step is itself iterative, as admins will continually conduct post-patch evaluations to improve success in the future.  



==> Text/Discussion.tex <==
\subsection{The Virtual Online Community of Practice of Patch Management}


The case we present here exhibits many of the same features observed in other literature, particularly around the collaboration aspects~\cite{kandogan2012taming, velasquez2008work, jenkins2020eurosp}.  Kandogan et al.~\cite{kandogan2012taming} makes continual references to the use of instant messengers, emails, or internal MOOs for sysadmins to confer, and cooperate towards finding a solution, yet the majority of their ethnographic studies primarily focus on their physical workplace. We extend on the work of Jenkins et al.~\cite{jenkins2020eurosp}, through detailing the collaborative efforts across online groups at the many stages of a single patches online life-cycle. 

We believe that it is valuable to study these collaborations in the online space as well, and adopt the notion of Virtual Community of Practice to frame our observations. 

Communities of practice~\cite{wenger1999communities} traditionally focus on people who interact regularly to learn together about a shared domain, which can range from producing new art to crisis management. We follow previous researchers~(e.g.~\cite{HaraHew:07,riverin2008sustaining}) in extending the notion of community of practice to online-only spaces. 

Here, our shared domain is patch management. However, these sysadmin VCOPs discussed have features which result in differing behaviours. Looking at patching under Microsoft's OS gives a 4 week routine imposed by Patch Tuesday, therefore we are in essence dealing with extremely quick and repetitive cycles of behaviour. These stages are repetitive, with information gathering for identification, followed by testing, reflective of the process described by participants in the work of Li et al~\cite{li2019keepers}. Contrasting this to the field of nursing, instead we have individual cases where the diseases or illnesses they discuss treatment option for, do not change as rapidly. Furthermore, in with nursing, usually it would be only one community member with direct access to a particular case. In our Sysadmins community, all patches are available to anyone, therefore we can receive much more technical, and customised advice 
%We have provided a detailed example of the types of behaviours exhibited in one of these virtual settings. We believe that our findings and the communities we have identified, are representative of an  

%Our work gives further credence to the original observation made by Kandogan et al. and in the context of patch management, the connection is more evident as to why these social systems are relied upon. 

\subsection{Signalling within VCOP}

Patching is a risk~\cite{beattie2002, shostack2003quantifying}, therefore any piece of information into the process is valuable and can aid in casting some light on the unknowns of patching, and therefore allow sysadmins to quantify the risks. Every member of the community has a differing experience and system, and therefore a different perspective, which enables them to learn and develop appropriate strategies for dealing with patches together. This triangulation of knowledge all focuses on the one problem: should I patch now?

Furthermore, we have detailed the extents of this behaviour and are able to see connections with that of Velasquez et al.~\cite{velasquez2008designing, velasquez2008sysadmins}, with the use of citations, screenshots, and detailed posts, blog or forum, we have essentially a form of information verification. This behaviour is reflective of Signalling, showing other community members that the information is real, important, and useful in their patching decisions. 
A number of qualities appear from our case study which illustrate this signalling behaviour, for example, the amount of detail given in attempts made to fix the issue, or the inclusion of log outputs, appear to be indicating to other members, ``Look, I ain't lazy, and this issue is real, I am worth helping!!''. Many admins are extremely busy, and therefore to receive help, you must demonstrate that you are worth helping, and that the issue is real. You must convince the community they too should be worried. 

This signalling behaviour is further instigated through information providence, in our case, sourcing and linking to multiple other ``respected'' news sources or forums. Here the number of posts are seen as an indicator that the problem is not unique and therefore may cause errors in a number of systems. Again, signalling is not restricted to the information shared, it is sometimes implicit given the advice the poster has shared. As with Woody's community, often the responses to advice or workarounds were reflective of their patching ``Philosophies'' (ie Group A, B, or W.). Moreover, these are framed as warnings regarding the advice they give, for example, Woody always seems to admit their advice is contrary to the vendor's advice, because at the end of the day, it is down to the individual sysadmin to make the decision on their system. 

Additionally, it allows those who perform the extra work to receive credit and build some social standing within the community. This compensates for the massive mount of person hours required for the invaluable sourcing of correct, timely information that is required due to the time-dependent nature of patching. 

\subsection{Trusting Vendors or Community}
Our findings demonstrate the complex trust dynamic which exists in patching between the consumer and the vendor. Takayama et al.~\cite{takayama2006trust}, showed that trust was a major factor in sysadmins preference for command line interfaces (CLI) over GUIs. It is clear from the responses following the pulling of the patch, that many sysadmins do not trust Microsoft, and this breakdown of trust has resulted from past bad experiences which have been discussed and shared within the Virtual Community of Practice, and are archived on their online sites. The effect of this breakdown of trust echoes the findings of Vaniea et al. \cite{vaniea2014} and Mathur et al.~\cite{mathur2016they} with end users, who take into account their relationship with a vendor and past bad experiences with updates.

Given the monthly cycles that MS patches experience, it appears that the recurring frustration prompt more apprehensive approaches to each patch, which is reinforced within 4 weeks with another Patch Tuesday. No piece of software is perfect from the offset, and therefore sysadmins may default to the easiest blanket strategies when dealing with patches; 1) Leave patching until errors are found, 2) If the patch causes error, then simply revert back and remove update. Our study indicates that in an uncertain patching landscape, these simple yet insecure policies, are the sanest option for sysadmins to follow. 


%discovered that end-users are also influenced through their relationship with the vendor. This dynamic is worth future focus as it appears that the opinions of some regarding the vendors in question, could steer the patch management strategies of many community members. 

We have discussed the work of many active members of the respective communities, and have not considered those who only consume and lurk~\cite{van20141}. Depending on the level that they consume this content from, they potentially miss out on exact details, but the communities use of blanket statements, such as the MS-DEFCON system could potentially influence their patching policies. This is an interesting avenue for future work, which could come to fruition in combination with the use of the WINE network \cite{dumitracs2011toward}. \adam{Remove this Paragraph?}

Updating, and updates in Windows, is a continually shifting environment, with the community having to adapt and adjust its practices as and when these changes occur. Moreover, in more recent indictments we have seen the power of the community, with calls for changes to the system being made through the participation of a survey and open letter from PatchManagement.org and Susan Bradley~\cite{openletter}. 
This community clearly wishes to be heard by Microsoft, and has the potential to shift Microsoft's patching strategies. 

\subsection{Limitations}

%The largest limitation of our work comes from the selection criteria for our patches. 
We specifically selected patches that exhibited multiple types of problems that admins must handle including: rare problems, a work around, a hotfix which also had problems, Microsoft pulling the hotfix, and a second hotfix. While we feel that these patches exemplify common patching situations that sysadmins must handle, we also acknowledge that it is uncommon for one patch to have this many issues associated with it. 
%While this is useful for our case study methodology, future work should focus on a comparative analysis Our patch selection may therefore have biased our results, though we also argue that this problem is a common one for case studies. 

A second limitation of our work is in how we found the posts and communities to analyze. We specifically started from the PatchManagement list and used the link structure in posts to find new relevant posts. While this approach allowed us to find all the information considered important enough to link to for our patches, it also excluded information that was less likely to be cited or simply not relevant for the patches we examined. 



==> Text/Introduction_old.tex <==
``Install updates in a timely manner'', is an example of security advice which is routinely shared with end-users, and championed by many within the security community~\cite{reeder2017152}. On the surface, this advice seems straightforward and less convoluted when compared to the many other pieces of advice which we are all exposed to. Yet, in the case of end-users, many have been shown to lack this awareness of the security critical nature of updating~\cite{vaniea2014,fagan2016they, redmiles2016learned, mathur2016they, forget2016or}. 

This observation can not, however, be applied to System Administrators (henceforth sysadmins) whose day-to-day tasks will include updating~\cite{velasquez2008designing}, while also juggling a number of diverse, complex, and highly collaborative IT maintenance tasks~\cite{barrett2004field,kandogan2012taming}. Sysadmins are aware both the risks of avoiding a patch, and the potential risks of patching~\cite{li2019keepers, shostack2003quantifying, tiefenau2020security}. Therefore, many may be motivated to simply ``wait it out'', as the errors and bugs of released patches are found and remedied, before deciding to patch~\cite{beattie2002}. 
This process is a potentially disastrous, as the release of patches is entangled with the disclosure of vulnerabilities, alerting nefarious actors of potential attack surfaces~\cite{bilge2012before}. We have seen infamous examples where this strategy of delay has caused massive damage to many such as the WannaCry attack on the NHS~\cite{lessonslearned}, and the Equifax data breach~\cite{goodin_2017_failure}. Furthermore, this time delay is relevant anywhere software is used, with patching reportedly taking between 45 days~\cite{nappa2015attack} to almost a full year for even just 50\% of devices to be secured in some instances. 

Deciding to patch hinges on balancing risk. Push a patch too early and you may inadvertently break business essential services. Push too late, and you may provide ample time for exploits to be developed and targeted at your systems. Identifying this optimum time is a difficult process for sysadmins~\cite{beattie2002}, requiring a number of stages and contextual information gathering to even consider patching~\cite{li2019keepers, tiefenau2020security, martiusdoes}. Nonetheless, we are left with a gap in our understanding: does this take so long? Or, where is this time spent, during the process of deciding to update? Hence, our research questions are:

[RQ1] How does the knowledge of risks associated with a patch develop over time?

[RQ2] How do the various communities support the collation and synthesizing of available

\hspace{24pt} information for sysadmins and other patching communities?


Given the clear dependence of sysadmins on both internal~\cite{kandogan2012taming} and external information sources~\cite{li2019keepers}, we address our research questions through an in-depth, descriptive case study to illuminate the online information life-cycle of two Microsoft patches. We track these patches across a number of online sources, from initial release to a final all-clear, ``time to patch'' announcement, almost a full month after release. Our case study highlights the scale of collaborative work found within and across communities of practice, which provides sysadmins with advice and data which is integral to deciding when to patch. Our case indicates areas where we could not only aid, but reduce the time necessary for information searching by  sysadmins needed for making their patching decisions.

We find that a number of information sources compile and collect knowledge from work performed elsewhere on the Internet. The use of forums and mailing lists also facilitates discussion and detective work that generates necessary information to inform patch decisions. These results reflect a number of individual Communities of Practice~\cite{wenger1999communities}, which collaborate to share knowledge and propagate information through out a wider Network of Practice~\cite{BrownJohnSeely2002Tslo}.

% \subsection{Research Questions}

% \begin{enumerate}
%  \item What does the information generated around a single issue look like?
%  \item How is information about patches presented and processed by key patch management communities? \\ (Things like announcements and collecting of data together into posts.)
% \item How does one key community's work, impact the information shared in another? \\
% (cross community data flow)
% \item What does "go wrong" look like in terms of information available online for sysadmins to make decisions based on? How does that information change over the course of a month?
% \item What do interactions look like between these communities and Microsoft? What information is Microsoft providing and how do communities use it? \\ (Quote, cite, ignore) 
% \item What does the information life cycle of a critical patch with a sleeper problem look like from an online-information perspective.
% \item What do interactions look like between these communities and Microsoft? What information is Microsoft providing and what complimentary information do communities generate? \\(Example of Known Issues being community sourced...)
% \item What role does time have in the process? \\(waiting on MS, waiting on community to test, to provide workarounds etc)
% \item What information blockers exist during the process, such as waiting for Microsoft to provide data, and others to post experiences.
% \item What is the time-related order to the available information? What info-sharing activities happen first, then second, and how does that flow impact information available to admins at different points?
% \item What shadow documentation are communities generating around MS patches and how is that documentation constructed?
% \item What information is necessary to convince a sysadmin community to patch?
% \item Where is the data initally posted??? 
% \item where does the information found within one community originate from? (official sources only or?)
% \item [Center nodes] often post announcements or collations of patching information, where do the content of these posts come from? 
% \item Admins (Influencers?) are expert information foragers, based on their community posts where and when are they getting access to patch-related data, and how do they express that data to others?
% \item What difficulties/barriers exist in information found within the breadth of sources available to admins? 
% \item What is slowing the timely availability of patch error information for admins?
% \item  What impact does time have on the type and accuracy of information available to admins?
% \item  In what ways does the information available to admins change over the the course of a patch month?
% \item What is the relationship between information availability and time look like for One Patch Incident?
% \item How do the known risks of a patching error develop over time?
% \item What events can influence the access to necessary information of a patch and it's risks? \\(security risks are known the whole way through, errors risk are slowly built up)
% \item At what point do the risks of patching no longer outweigh the risks of not patching?
% \item What information flow blockers exist during the process? Such as waiting on official announcements, 
%  such as waiting for Microsoft to provide data, information being in disparate locations, and others to post experiences.
%  \item What prevents these risks from being identified earlier?
%  \item 
%  \item What enables new information flow into the community? Such as: announcements from MS, information from members' tests, links to information in other communities. 
%  \item How do the various communities support the collation and synthesizing of available information for their members?
%  \item how do different can a single communities situational awareness differ from/depend on another?
%  \item Given the breadth of Information sources available to sysadmins, how do they compliment one another? Do some sources produce only certain types of patch information. (Announcement release -> Security Lists -> Errors -> Announcement observations/Vendor awareness -> repeat for hotfix) 
% \item given RQ1: What information generators/source/ can exits and how do they contribute to this developing understanding of risks?
% \item What 'unofficial' sources contribute to a patch risk understanding? and How do these sources collaborate and share their information?
% \item how do distinct sources collectively contribute to this knowledge 
% \item How do different communities contribute and derive benefit from these cross community collaborations?
% \end{enumerate}





%Though the importance of updating is known within the security community\cite{reeder2017152}, system administrators (henceforth sysadmins) do not always immediately update when patches become available, even if the vendor labels them as security critical. Sometimes, delaying an update is the correct decision, because a patch might break critical functionality. However, in the worst case, this can lead to severe disruption. A case in point is the famous attack by the ransomware WannaCry~\cite{lessonsLearned}, which severely disrupted the services of at least 34\% of NHS England Trusts~\cite{nationalauditoffice_2017}.

%It is sysadmins who are responsible for patch management~\cite{velasquez2008designing}. The role of sysadmins is varied, complex, and dynamic, as they juggle multiple systems, virtual and physical, while considering the needs of their employer~\cite{barrett2004field, kandogan2012taming}. Existing literature suggests that sysadmins' decisions often involve complex, time-dependent~\cite{bilge2012before} risk calculation~\cite{beattie2002, shostack2003quantifying}.  This leads to the question: How do sysadmins manage patches, and what are the risks that would lead sysadmins to delay installing a patch? 

%Since there is relatively little literature on patch management decisions, with some exceptions~\cite{furnell2016vulnerability}, we decided to investigate the journey of a patch from release to installation in a detailed case study of two critical Microsoft patches, KB4034679 and KB4034664, which were released on August 8, 2017. In our analysis, we focus on a virtual community of practice of sysadmins spread across several forums, blogs, and mailing lists that performs detailed risk assessments of patches as they are released, and as patches to these patches are published. We map out key contexts and influencers, and describe how sysadmins with different risk tolerance profiles use the information to decide whether they can risk applying a patch.   



%and is part of the UK Government's advised  ``Cyber Essentials''~\footnote{\url{https://www.ncsc.gov.uk/scheme/cyber-essentials}}, these events lead many to question the state of patch management\cite{furnell2016vulnerability}. However, in the case outlined above, we are not talking about end-users; instead we are looking at IT infrastructure personnel, or System Administrators (sysadmins henceforth). 
%Given the global impact of these events, a simple question arose in our minds; how do sysadmins make decisions around which patch to install?


%At 13:00, on the 12th of May, 2017, the UK's National Health Service (NHS) Digital's CareCERT issued an alert to the Department of Health and Social Care (DHSC). The alert detailed that four Trusts from across England were reporting that their IT services were being held ransom. By 16:00, the number of trusts reporting of the attack had quadrupled~\cite{lessonsLearned}. 
%This was WannaCry, a preventable ransomware attack from which the impact could be felt across the globe. In the following six days, at least 34\% of NHS England Trusts experienced disruption to their service provision, which was estimated to equate to 19,494 cancelled appointments, which included patient operations~\cite{nationalauditoffice_2017}. This incident brought to light the frailties of current patching methods, and in fact lessons were not immediately learned as less than two moths later NotPetya hit, which used the same vulnerabilty as WannaCry and caused over \$300 million in damages for Mersck alone \cite{someNews}.
%The lesson learned by many following this international event was that updates and updating software is a critical security mechanism that must be followed, and is now advised as part of the UK Government's ``Cyber Essentials''~\footnote{\url{https://www.ncsc.gov.uk/scheme/cyber-essentials}} scheme for large organizations and SMEs.


%The role of sysadmins is varied, complex, and dynamic - as they juggle multiple systems, virtual and physical, while considering the needs of their employer~\cite{barrett2004field, kandogan2012taming},  however patch management is one task which remains consistent to all sysadmins The distinctive difficulties this role can raise is more apparent when we consider patch management, Given the insufficient amount of academic literature on the subject, our research intends to fill this gap. 

%In this paper, we present a case study of two critical Microsoft patches, and how online sysadmin communities reacted to the them from release to the declaring them safe to install. We map out key contexts and influencers, and discuss potential theoretical frameworks for our findings, which can then be used to develop further avenues of work. 
%We conclude with further  provide context through literature and map out the setting for our case. We will end with a discussion of our work and highlight future avenues which can be built upon following our case findings. 

%  One such example which highlights the complexities associated with the role is that of Patch Management - the process of applying code changes to systems and software. The task of patch management can involve several sub-tasks such as discovering a patch exists, obtaining it, testing for problems, and applying it to many systems. Furthermore, sysadmins must maintain their current knowledge of available patches in conjunction with knowledge of their systems. This information is highly influential in sysadmins decision processes as it is utilised to perform risk management. Through collaboration, sysadmins accumulate and distribute information seen to aid in this decision process. The risks they are balancing include the vulnerability of their systems, the usability of post-patched their systems for end-users and the goals of the organisation. 
 %Patches and updates are rarely straightforward, as patches to systems can result in unintentional consequences, such as the breakdown of essential systems. Therefore, information-seeking is vital and has spawned large communities of collaborative sysadmins, as they work together to construct a shared understanding of the risks associated with various patches. 
 
 %Such discussions were found to take place across multiple communication platforms, with the community actively working to disseminate information quickly. Collaborative accumulation of information underlines the significance of patch related information and emphasises the scale of people-hours poured into this shared task. Threads and discussions are built upon by numerous sysadmins, calling on individual experience, knowledge, and evidence -- which is in turn distributed across forums or mailing lists. Sysadmins then draw from these various information sources to investigate their own systems' context. This results in an unofficial Information Economy that influences the decision processes of those involved. This crowd-sourced data collection and discussion creates self assigned roles within the community to ensure the overall success of the Windows patch management process. 
 
% From our research we can see evidenced the role of Social Influencers within these communities, the extent of the influence that they have over numerous sysadmins and their respective systems. Furthermore, this collaborative effort can be used to provide feedback to Microsoft, primarily to raise their awareness of issues and justify a response from Microsoft.

%% Need to streamline this - still alot I want to say, such as the importance of Patching. Complexities of systems, one glove does not fit all, but through drawing from multiple perspectives and skills sets, one can get a better understanding of a situation and its possible risk to themselves. Should talk more about WannaCry, CodeRed.... why not install the update? whats going on here?
